Augmenting Chest X-ray Datasets with Non-Expert Annotations

The advancement of machine learning algorithms in medical image analysis requires the expansion of training datasets. A popular and cost-effective approach is automated annotation extraction from free-text medical reports, primarily due to the high costs associated with expert clinicians annotating medical images, such as chest X-rays. However, it has been shown that the resulting datasets are susceptible to biases and shortcuts. Another strategy to increase the size of a dataset is crowdsourcing, a widely adopted practice in general computer vision with some success in medical image analysis. In a similar vein to crowdsourcing, we enhance two publicly available chest X-ray datasets by incorporating non-expert annotations. However, instead of using diagnostic labels, we annotate shortcuts in the form of tubes. We collect 3.5k chest drain annotations for NIH-CXR14, and 1k annotations for four different tube types in PadChest, and create the Non-Expert Annotations of Tubes in X-rays (NEATX) dataset. We train a chest drain detector with the non-expert annotations that generalizes well to expert labels. Moreover, we compare our annotations to those provided by experts and show "moderate" to "almost perfect" agreement. Finally, we present a pathology agreement study to raise awareness about the quality of ground truth annotations. We make our dataset available on Zenodo at https://zenodo.org/records/14944064 and our code available at https://github.com/purrlab/chestxr-label-reliability.

==> figures/fig_chest_xrays_old.tex <==
\begin{figure}
  \centering
  \begin{tabular}{ c @{\hspace{20pt}} c }
    \includegraphics[width=.4\columnwidth]{images/A-chest-drain.png} &
      \includegraphics[width=.4\columnwidth]{images/B-tracheostomy.png} \\
    \small (a) Chest drain &
      \small (b) Tracheostomy \\
    \includegraphics[width=.4\columnwidth]{images/C-NSG.png} &
      \includegraphics[width=.4\columnwidth]{images/D-endo.png} \\
    \small (c) NSG - Nasogastric  &
      \small (d) Endotracheal
  \end{tabular}
  \medskip
  \caption{Tube examples in \padchest{} dataset.}
  \label{fig:chest-xray-tubes}
\end{figure}

==> tables/table_multitask.tex <==
\begin{table*}[t] 
    \centering
    \begin{tabular}{lcccccccc}
    \toprule
     & \textbf{Effusion} & \textbf{Pneumothorax} & \textbf{Atelectasis} & \textbf{Cardiomegaly} & \textbf{Pneumonia} \\ [0.5ex]
    \midrule
    Single & 94.2 $\pm$ 0.1 & 81.4 $\pm$ 2.3 & \textbf{86.9}  $\pm$ 0.1 &  89.2 $\pm$ 0.2 & 81.0 $\pm$ 0.3 \\
    Multitask & \textbf{94.3} $\pm$ 0.1 & \textbf{84.2} $\pm$ 0.8 & 86.8 $\pm$ 0.3 & \textbf{89.4} $\pm$ 0.1 & 80.1 $\pm$ 0.5 \\
    \bottomrule
    \end{tabular}
    \vspace{5pt}
    \caption{Results on the pathology detection task in \padchest{}. We report the average AUC $\pm$ standard deviation over three model runs. We mark the highest average AUC obtained for each pathology in bold.}
    \label{tab:multitask}
\end{table*}

